Optimal Caching and Routing in Hybrid Networks

Hybrid networks consisting of MANET nodes and cellular infrastructure have been recently proposed to improve the performance of military networks. Prior work has demonstrated the benefits of in-network content caching in a wired, Internet context. We investigate the problem of developing optimal routing and caching policies in a hybrid network supporting in-network caching with the goal of minimizing overall content-access delay. Here, needed content may always be accessed at a back-end server via the cellular infrastructure; alternatively, content may also be accessed via cache-equipped "cluster" nodes within the MANET. To access content, MANET nodes must thus decide whether to route to in-MANET cluster nodes or to back-end servers via the cellular infrastructure; the in-MANET cluster nodes must additionally decide which content to cache. We model the cellular path as either i) a congestion-insensitive fixed-delay path or ii) a congestion-sensitive path modeled as an M/M/1 queue. We demonstrate that under the assumption of stationary, independent requests, it is optimal to adopt static caching (i.e., to keep a cache's content fixed over time) based on content popularity. We also show that it is optimal to route to in-MANET caches for content cached there, but to route requests for remaining content via the cellular infrastructure for the congestion-insensitive case and to split traffic between the in-MANET caches and cellular infrastructure for the congestion-sensitive case. We develop a simple distributed algorithm for the joint routing/caching problem and demonstrate its efficacy via simulation.

==> cent_algo.tex <==
\section{Centralized Algorithms}
\label{sec:cent_soln}
We assume that there is a centralized agent which takes routing decisions on behalf of the users. The users route all requests to the centralized agent which  either forwards the request to the cache or informs the users to route through 4G. The centralized agent can adopt static caching where it determines the overall popularity of files and caches the most popular ones.  Static caching can be  hard to implement in practice because file popularity can change over time.  A classic caching policy such as LRU adapts itself to changing  file popularity but does not perform as well as static caching when popularity does not change or changes very slowly over time.  Recently 2-LRU caching policy has been proposed by \cite{Martina14} which gives good performance in both scenarios. We propose the use of a caching policy similar to 2-LRU for the centralized algorithm.

\subsection{2 -LRU}
 The 2-LRU caching policy adopted from \cite{Martina14} works as follows. There are 2 caches, the first cache is an id cache which receives all requests and functions as a regular LRU cache. The second cache is the main content cache and it receives  requests as forwarded by the id cache. For all  requests that the main content cache receives it functions as a LRU cache. We assume that the id cache is present at the centralized agent. We also assume that the centralized agent fakes the content cache in the sense that it keeps a virtual content cache as well to keep track of what files are actually present in the content cache. 

The  id cache receives all requests. If the request is a hit in  the id cache it is forward to the main content cache. If the item is present in the content cache, it is a hit and the request is served to the user, otherwise it is a miss. When the request is a miss, the main content cache obtains the  content,  replaces files according to the LRU policy and serves the user. The virtual content cache which is maintained at the centralized agent is also updated, so that the agent is aware of  the actual state of the content cache. When the request is a miss in the id cache, the central agent checks in the virtual content cache to see if the item is present. If it a item is present in the virtual content cache, the request is forwarded to the main content cache. The requested file is returned to the user and the time stamp for the file is updated in both the main content and virtual content caches. If  the request is a miss in the id cache and the item is not present in the virtual content cache, the central agent requests the user to route through the 4G path. Figure \ref{fig:centralized_agent} shows the working of the system. 

\begin{figure} [ht]
  \begin{center}
  \includegraphics[width = 3.0in, height = 2.0in]{./Figures/central_agent.png}
  \caption{Central Agent}
  \vspace{-0.5cm}
    \label{fig:centralized_agent}
  \end{center}
\end{figure}


\subsection{$\alpha$ 2 -LRU}
One can adopt the 2-LRU caching policy unchanged when the delay through the 4G path is constant. However when the 4G path is modeled as a queuing system (we assume it is M/M/1), it may not be possible to send all requests that miss both the id and the main cache through the 4G as it can increase the user delay.  For this reason we propose $\alpha$ 2-LRU policy in which when the request is a miss in both the id and the content cache, with probability $\alpha$, the request is still forwarded to the content cache and  with probability $(1 -\alpha)$, the request is sent through the 4G path. 

We next analytically model the functioning of an $\alpha$ 2 -LRU cache.  In \cite{Martina14}, the authors develop a Markov chain model to describe the functioning of a 2-LRU cache. We augment this Markovian model to model the functioning of an $\alpha$ 2 -LRU cache. The Markovian model is shown in figure \ref{fig:markov_chain_alpha}. It is easy to determine the steady state probabilities of this Markov chain.
\\ $\pi_{0,0} = \frac{q_b}{1 - (1-\alpha)q_c}$
\\ $\pi_{1,0} = \frac{ (1-\alpha)q_a q_b}{1- (1-\alpha)q_c}$
\\ $\pi_{0,1} = q_c(1- \frac{ (1-\alpha)q_b}{1- (1-\alpha)q_c})$
\\ $\pi_{1,1} = q_a(1- \frac{ (1-\alpha)q_b}{1- (1-\alpha)q_c})$

Let $p_{hit}$, $p_{miss}$ and $p_{4G}$  denote the hit probability, the miss probability and  the 4G access probability respectively. Therefore,
\\ $p_{hit} = \pi_{0,1}  + \pi_{1,1} $
\\ $p_{miss} = \alpha \pi_{0,0}  + \pi_{1,0} $ 
\\$p_{4G}  = (1 -\alpha)\pi_{0,0}$.

\begin{figure} [ht]
  \begin{center}
  \includegraphics[width = 3.0in, height = 2.0in]{./Figures/Markov.png}
  \caption{Markov Chain for  $\alpha$ 2 -LRU}
  \vspace{-0.5cm}
    \label{fig:markov_chain_alpha}
  \end{center}
\end{figure}


Figure \ref{fig:alpha_2LRU} shows how the hit, miss and access probabilities change  with varying  $\alpha$. We  observe from the figure that the simulation and model results match each other closely.

\begin{figure} [ht]
  \begin{center}
  \includegraphics[width = 3.0in, height = 2.0in]{./Figures/TwoLRU_alpha_hits_MM1.png}
  \caption{Variation of Hit/Miss/Access probability for  $\alpha$ 2 -LRU}
  \vspace{-0.5cm}
    \label{fig:alpha_2LRU}
  \end{center}
\end{figure}



\subsection{ Optimal $\alpha$ 2 -LRU and Optimal sized id cache 2-LRU}
In order for the  $\alpha$ 2 -LRU caching policy to work well in the presence of an M/M/1 queue 4G path, we have to choose the  optimal value of $\alpha$. The optimal value of $\alpha$ is determined by minimizing the total delay experienced by the user under the $\alpha$ 2 -LRU caching policy (\blue{Expression not given here}). The value of alpha is mainly dependent on the service capacity of the M/M/1 queue and the aggregate traffic arriving at the central agent.

A similar effect of allowing more traffic through the cache as achieved by the $\alpha$ 2 -LRU caching policy can also be obtained by changing the size of the id cache. Note that in \cite{Martina14}, the authors assume that the size of the id and the content cache is the same. {\it Optimal sized id cache} 2-LRU determines the optimal size of the id cache given the service capacity and the  aggregate traffic arriving at the central agent.  The optimal size of id cache  is determined by minimizing the total delay experienced by the user (\blue{ the Markov chain and the corresponding expression are available in \cite{Martina14}}).

Figure \ref{fig:alpha_2LRU_vs_side_cache} compares the performance (numerically) of static caching (shown to be optimal in section V.B), optimal $\alpha$ 2 -LRU and {\it optimal sized id cache} 2-LRU under IRM traffic with Zipf popularity distribution. We  observe  from the figure that the performance of the optimal $\alpha$ 2 -LRU and {\it optimal sized id cache} 2-LRU is close to optimal static caching with {\it optimal sized id cache} 2-LRU caching outperforming  optimal $\alpha$ 2 -LRU.


\begin{figure} [ht]
  \begin{center}
  \includegraphics[width = 3.0in, height = 2.0in]{./Figures/Static_vs_Side_Alpha.png}
  \caption{Performance Comparison: Static,  Optimal $\alpha$ 2 -LRU, Optimal sized id cache 2-LRU  }
  \vspace{-0.5cm}
    \label{fig:alpha_2LRU_vs_side_cache}
  \end{center}
\end{figure}



